SS5G: Collision Resolution Protocol for Delay and Energy Efficient LoRa Networks

Future 5G and Internet of Things (IoT) applications will heavily rely on long-range communication technologies such as low-power wireless area networks (LPWANs). In particular, LoRaWAN built on LoRa physical layer is gathering increasing interests, both from academia and industries, for enabling low-cost energy efficient IoT wireless sensor networks for, e.g., environmental monitoring over wide areas. While its communication range may go up to 20 kilometers, the achievable bit rates in LoRaWAN are limited to a few kilobits per second. In the event of collisions, the perceived rate is further reduced due to packet loss and retransmissions. Firstly, to alleviate the harmful impacts of collisions, we propose a decoding algorithm that enables to resolve several superposed LoRa signals. Our proposed method exploits the slight desynchronization of superposed signals and specific features of LoRa physical layer. Secondly, we design a full MAC protocol enabling collision resolution. The simulation results demonstrate that the proposed method outperforms conventional LoRaWAN jointly in terms of system throughput, energy efficiency as well as delay. These results show that our scheme is well suited for 5G and IoT systems, as one of their major goals is to provide the best trade-off among these performance objectives.

==> biblio <==
@inproceedings{elrachkidy18decoding,
    author = {El Rachkidy, N. and Guitton, A. and Kaneko, M.},
    title = {Decoding Superposed {L}o{R}a Signals},
    booktitle = {IEEE Local Computer Networks (LCN)},
    year = {2018},
}

@techreport{lora,
    author = {{Semtech Corporation}},
    title = {{AN1200.22 LoRa Modulation Basics}},
    institution = {Semtech},
    number = {Revision 2},
    type = {Application note},
    note = {accessed 2018-01-29},
    url = {http://www.semtech.com/uploads/documents/an1200.22.pdf},
    year = {2015},
}

@inproceedings{toussaint16performance,
	author = {Toussaint, J. and El Rachkidy, N. and Guitton, A.},
	title = {Performance analysis of the on-the-air activation in {LoRaWAN}},
	booktitle = {{IEEE} {I}nformation {T}echnology, {E}lectronics and {M}obile {C}ommunication {C}onference ({IEMCON})},
	year = {2016},
}

@inproceedings{margelis15low,
	author = {Margelis, G. and Piechocki, R. and Kaleshi, D. and Thomas, P.},
	title = {Low Throughput Networks for the {I}o{T}: Lessons learned from industrial implementations},
	booktitle = {IEEE World Forum on Internet of Things (WF-IoT)},
	pages = {181--186},
	year = {2015},
}

@techreport{3gpp,
	author = {3GPP},
	title = {Cellular system support for ultra-low complexity and low throughput {I}nternet of {T}hings ({CI}o{T})},
	type = {Technical report},
	number = {45.820},
	institution = {3rd Generation Partnership Project (3GPP)},
	year = {2015},
}

@Inbook{vangelista15long,
	author = {Vangelista, L. and Zanella, A. and Zorzi, M.},
	title = {Long-Range {I}o{T} Technologies: The Dawn of {L}o{R}a{\texttrademark}},
	bookTitle = {Future Access Enablers for Ubiquitous and Intelligent Infrastructures: First International Conference (FABULOUS) - revised selected papers},
	year = {2015},
	publisher = {Springer International Publishing},
	pages = {51--58},
	isbn = {978-3-319-27072-2},
	doi = {10.1007/978-3-319-27072-2_7},
}

@article{goursaud15dedicated,
	TITLE = {Dedicated networks for {I}o{T}: {PHY} / {MAC} state of the art and challenges},
	AUTHOR = {Goursaud, C. and Gorce, J.-M.},
	JOURNAL = {EAI endorsed Transactions on {I}nternet of {T}hings},
	YEAR = {2015},
	DOI = {10.4108/eai.26-10-2015.150597},
	HAL_ID = {hal-01231221},
}

@article{song16survey,
	author = {Song, Q. and Nuaymi, L. and Lagrange, X.},
	title = {Survey of radio resource management issues and proposals for energy-efficient cellular networks that will cover billions of machines},
	journal = {{EURASIP} {J}ournal on {W}ireless {C}ommunications and {Network}},
	pages = {1-20},
	year= {2016},
}

@techreport{etsi12electromagnetic,
	author = {{ETSI}},
	title = {Electromagnetic compatibility and radio spectrum matters ({ERM}); Short Range Devices ({SRD}); Radio equipment to be used in the 25 {MHz} to 1000 {MHz} frequency range with power levels ranging up to 500 {mW}; Part 1: Technical characteristics and test methods},
	institution = {ETSI},
	type = {EN},
	number = {300 220-1 v2.4.1},
	year = {2012},
	month = {05},
}

@techreport{semtech15lora,
	author = {Semtech},
	title = {Lo{R}a\textsuperscript{{\tiny TM}} Modulation Basics},
	institution = {Semtech Corporation},
	year = {2015},
	month = {May},
	type = {application note},
	number = {1200.22},
	note = {revision 2},
}

@techreport{libelium15waspmote,
	author = {Libelium},
	title = {Waspmote {L}o{R}a 868 {MH}z 915 {MH}z {SX}1272 Networking Guide},
	institution = {Libelium Comunicaciones Distribuidas S. L.},
	year = {2015},
	month = {November},
	note = {version 4.2},
}

@techreport{sx1272,
    author = {{Semtech Corporation}},
    title = {{SX1272/73} - 860 {MH}z to 1020 {MH}z {L}ow {P}ower {L}ong {R}ange {T}ransceiver},
    institution = {Semtech Corporation},
    note = {Rev. 3.1},
    month = {March},
    year = {2017},
}

@inproceedings{ngangue09analytical,
	author = {Ngangue Ndih, E. D. and Khaled, N. and De Micheli, G.},
	title = {An analytical model for the contention access period of the slotted {IEEE} 802.15.4 with service differentiation},
	booktitle = {IEEE International Conference on Communications (ICC)},
	year = {2009},
}

@inproceedings{park09generalized,
	author = {Park, P. and Di Marco, P. and Soldati, P. and Fischione, C. and Johansson, K. H.},
	title = {A generalized {M}arkov chain model for effective analysis of slotted {IEEE} 802.15.4},
	booktitle = {IEEE International Conference on Mobile Adhoc and Sensor Systems (MASS)},
	year = {2009},
}

@article{striccoli14markov,
	author = {Striccoli, D. and Boggia, G. and Grieco, L. A.},
	title = {A {M}arkov model for characterizing {IEEE} 802.15.4 {MAC} layer in noisy environments},
	journal = {IEEE Transactions on Industrial Electronics},
	year = {2014},
}

@inproceedings{tao06performance,
	author = {Tao, Z. and Panwar, S. and Gu, D. and Zhang, J.},
	title = {Performance analysis and a proposed improvement for the {IEEE} 802.15.4 contention access period},
	booktitle = {IEEE Wireless Communications and Networking Conference (WCNC)},
	year = {2006},
}

@inproceedings{xiao11analytical,
	author = {Xiao, Z. and He, C. and Jiang, L.},
	title = {An analytical model for {IEEE} 802.15.4 with sleep mode based on time-varying queue},
	booktitle = {IEEE International Conference on Communications (ICC)},
	year = {2011},
}

@article{centenaro16long,
	author = {Centenaro, M. and Vangelista, L. and Zanella, A. and Zorzi, M.},
	title = {Long-range communications in unlicensed bands: the rising stars in the {I}o{T} and smart city scenarios},
	journal = {IEEE Wireless Communications},
	year = {2016},
}

@techreport{802-15-4-2003,
	author = {{IEEE 802.15}},
	title = {Part 15.4$\colon$ Wireless Medium Access Control ({MAC}) and Physical Layer ({PHY}) Specifications for Low-Rate Wireless Personal Area Networks ({LR-WPAN}s)},
	institution = {ANSI/IEEE},
	type = {Standard 802.15.4},
	number = {R2003},
	year = {2003},
}

@techreport{802-15-4-2006,
	author = {{IEEE 802.15}},
	title = {Part 15.4$\colon$ Wireless Medium Access Control ({MAC}) and Physical Layer ({PHY}) Specifications for Low-Rate Wireless Personal Area Networks ({WPAN}s)},
	institution = {ANSI/IEEE},
	type = {Standard 802.15.4},
	number = {R2006},
	year = {2006},
}

@techreport{802-15-4-2011,
	author = {{IEEE 802.15}},
	title = {Part 15.4$\colon$ Low-Rate Wireless Personal Area Networks ({LR}-{WPAN}s)},
	institution = {IEEE},
	type = {Standard for local and metropolitan area networks},
	number = {IEEE Std 802.15.4-2011},
	year = {2011},
}

@techreport{lorawan-2015,
	author = {Sornin, N. and Luis, M. and Eirich, T. and Kramp, T. and Hersent, O.},
	title = {{L}o{R}a{WAN} {S}pecification},
	institution = {LoRa Alliance},
	type = {Standard},
	number = {V1.0},
	year = {2015},
}

@techreport{lorawan-2017,
    author = {{LoRa Alliance Technical Committee}},
    title = {{LoRaWAN 1.1 Specification}},
    institution = {LoRa Alliance},
    type = {Standard},
    number = {V1.1},
    year = {2017},
}

@techreport{lorawan-regional-settings-2017,
    author = {{LoRa Alliance Technical Committee}},
    title = {{LoRaWAN 1.1 Regional Parameters}},
    type = {Standard},
    number = {V1.1, Revision A},
    year = {2017},
}

@article{oliveira11wireless,
	author = {Oliveira, L. M. L.},
	title = {{W}ireless {S}ensor {N}etworks: a {S}urvey on {E}nvironmental {M}onitoring},
	journal = {Journal of communications},
	volume = {6},
	number = {2},
	year = {2011},
}

@article{yick08wireless,
	author = {Yick, J. and Mukherjee, B. and Ghosal, D.},
	title = {Wireless sensor network survey},
	journal = {Computer Networks},
	volume = {52},
	number = {12},
	pages = {2292--2330},
	year = {2008},
}

@misc{sigfox,
	author = {Sigfox},
	note = {http//www.sigfox.com},
}

@misc{ingenu,
	author = {Ingenu},
	note = {http//www.ingenu.com},
}

@article{fafoutis14harvesting,
	author = {Fafoutis, X. and Sorensen, T. and Madsen, J.},
	title = {Energy {H}arvesting - {W}ireless {S}ensor {N}etworks for {I}ndoors {A}pplications {U}sing {IEEE} 802.11},
	journal = {Procedia Computer Science},
	publisher = {Elsevier},
	volume = {32},
	pages = {991--996},
	year = {2014},
}

@inproceedings{rohokale11cooperative,
	author = {Rohokale, V. M. and Prasad N. R. and Prasad, R.},
	title = {A cooperative {I}nternet of {T}hings {(IoT)} for rural healthcare monitoring and control},
	booktitle = {Wireless Communication, Vehicular Technology, Information Theory and Aeroscpace Electronic Systems Technology (Wireless ViTAE), 2001, 2nd Internal Conference on},
	pages = {1--6},
	year = {2011},
}

@article{zanella14internet,
	author = {Zanella, A. and and Bui, N. and Castellani, A. and Vangelista, L. and Zorzi, M.},
	title = {Internet of {T}hings for {S}mart {C}ities},
	journal = {{IEEE} {I}nternet of {T}hings {J}ournal},
	volume = {1},
	pages = {22-32},
	year= {2014},
}

@article{petajajarvi17evaluation,
    author = {Pet\"aj\"aj\"arvi, J. and Mikhaylov, K. and Yasmin, R. and H\"am\"al\"ainen, M. and Iinatti, J.},
    title = {Evaluation of {LoRa} {LPWAN} technology for indoor remote health and wellbeing monitoring},
    journal = {International Journal of Wireless Information Networks},
    volume = {24},
    number = {2},
    pages = {153--165},
    year = {2017},
}

@inproceedings{nolan16evaluation,
    author = {Nolan, K. E. and Guibene, W. and Kelly, M. Y.},
    title = {An evaluation of low power wide area network technologies for the {I}nternet of {T}hings},
    booktitle = {International Wireless Communications and Mobile Computing Conference (IWCMC)},
    pages = {439--444},
    journal = {2016},
}

@article{haxhibeqiri17lora,
    author = {Haxhibeqiri, J. and Van den Abeele, F. and Moerman, I. and Hoebeke, J.},
    title = {{L}o{R}a scalability: a simulation model based on interference measurements},
    journal = {Sensors},
    publisher = {MDPI},
    volume = {17},
    number = {6},
    pages = {1193},
    year = {2017},
}

@inproceedings{croce17impact,
    author = {Croce, D. and Gucciardo, M. and Tinnirello, I. and Garlisi, D. and Mangione, S.},
    title = {Impact of spreading factor imperfect orthogonality in {L}o{R}a communications},
    booktitle = {International Tyrrhenian Workshop on Digital Communication (TIWDC)},
    series = {Communications in Computer and Information Science (CCIS)},
    pages = {165--179},
    volume = {766},
    year = {2017},
}

@inproceedings{zhu18evaluation,
    author = {Zhu, G. and Liao, C.-H. and Suzuki, M. and Narusue, Y. and Morikawa, H.},
    title = {Evaluation of {L}o{R}a receiver performance under co-technology interference},
    booktitle = {IEEE Consumer Communications and Networking Conference (CCNC)},
    year = {2018},
}

@INPROCEEDINGS{Karkatis16demyst,
    AUTHOR = "{S. Kartakis, B.D. Choudhary, A.D. Gluhak, L. Lambrinos and J.A. McCann}",
    TITLE = "{Demystifying low-power wide-area communications for city IoT applications}",
    BOOKTITLE = "{ACM} {Tenth ACM International Workshop on Wireless Network Testbeds, Experimental Evaluation, and Characterization (WiNTECH '16)}", 
    YEAR = "2016",
    address = "NYC, New York",
    month = "October",
    file = F
}

@ARTICLE{Raza17low,
  AUTHOR =       "{U. Raza, P. Kulkarni, R. Xu and M. Sooriyabandara}",
  TITLE =        "{Low Power Wide Area Networks: an Overview}",
  JOURNAL =      "{IEEE Communications Surveys and Tutorials}",
  YEAR =         "2017",
  volume =       "19",
  number =       "2",
  pages =        "855-873",
  month =        "January",
  file = F
}

@ARTICLE{Xiong15low,
  AUTHOR =       "{X. Xiong, K. Zheng, R. Xu, W. Xiang and P. Chatzimisios}",
  TITLE =        "{Low Power Wide Area Machine-to-Machine Networks: Key Techniques and Prototype}",
  JOURNAL =      "{IEEE Communications Magazine}",
  YEAR =         "2015",
  volume =       "53",
  number =       "9",
  pages =        "64-71",
  month =        "September",
  file = F
}


@MISC{Waret18LoRa,
	AUTHOR =       "{A. Waret, M. Kaneko, A. Guitton and N. El Rachkidy}",
	Title          = "{LoRa Throughput Analysis with Imperfect Spreading Factor Orthogonality}",
    	Howpublished   = "arXiv:1803.06534 [cs.NI]",
    	Year           = "2018",
    	file = F
}


@ARTICLE{Geo17apr,
  AUTHOR =       "{O. Georgiou and U. Raza}",
  TITLE =        "{Low Power Wide Area Network Analysis: Can LoRa Scale?}",
  JOURNAL =      "{IEEE Wirel. Commun. Letters}",
  YEAR =         "2017",
  volume =       "6",
  number =       "2",
  pages =        "162-165",
  month =        "April",
  file = F
}


@INPROCEEDINGS{Bor16nov,
    AUTHOR = "{M. Bor, U. Roedig, T. Voigt and J.M. Alonso}",
    TITLE = "{Do LoRa Low-Power Wide-Area Networks Scale?}",
    BOOKTITLE = "{ACM} {MSWiM}", 
    YEAR = "2016",
    address = "Malta",
    month = "November",
    file = F
}


@article{Lim18spreading,
	TITLE = {{Spreading Factor Allocation for Massive Connectivity in LoRa Systems}},
	AUTHOR = {J.T. Lim and Y. Han}, 
	JOURNAL = {IEEE Communications Letters},
	YEAR = {2018},
	volume =  "22",
  	number =  "4",
  	pages =  "800-803",
	month =  "April",
	DOI = {},
	HAL_ID = {},
}

@inproceedings{Reynders17power,
	author = {B. Reynders, W. Meert and S. Pollin},
	title = {Power and Spreading Factor Control in Low Power Wide Area Networks},
	booktitle = {{IEEE} International Conference on Communications (ICC)},
	year = {2017},
}

@inproceedings{Qin17spreading,
	author = {Z. Qin and J. A. McCann},
	title = {{Resource Efficiency in Low-Power Wide-Area Networks for IoT Applications}},
	booktitle = {{IEEE} Global Communications Conference (Globecom)},
	year = {2017},
}

